Weakly-Supervised Cloud Detection with Fixed-Point GANs

The detection of clouds in satellite images is an essential preprocessing task for big data in remote sensing. Convolutional neural networks (CNNs) have greatly advanced the state-of-the-art in the detection of clouds in satellite images, but existing CNN-based methods are costly as they require large amounts of training images with expensive pixel-level cloud labels. To alleviate this cost, we propose Fixed-Point GAN for Cloud Detection (FCD), a weakly-supervised approach. Training with only image-level labels, we learn fixed-point translation between clear and cloudy images, so only clouds are affected during translation. Doing so enables our approach to predict pixel-level cloud labels by translating satellite images to clear ones and setting a threshold to the difference between the two images. Moreover, we propose FCD+, where we exploit the label-noise robustness of CNNs to refine the prediction of FCD, leading to further improvements. We demonstrate the effectiveness of our approach on the Landsat-8 Biome cloud detection dataset, where we obtain performance close to existing fully-supervised methods that train with expensive pixel-level labels. By fine-tuning our FCD+ with just 1% of the available pixel-level labels, we match the performance of fully-supervised methods.

==> BigData 2021 Weakly-Supervised Cloud Detection with Fixed-Point GANs/figures/predictions_full.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{images/predictions_zoom.pdf}
%    \includegraphics[width=0.8\linewidth,trim=0 0 0 62, clip]{images/predictions_full.pdf}
    \caption{Example cloud mask results of FCD and FCD+ on Landsat-8 images from each biome.}
    \label{fig:predictionsfull}
\end{figure*}

==> BigData 2021 Weakly-Supervised Cloud Detection with Fixed-Point GANs/figures/predictions_zoom.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\linewidth]{images/predictions_zoom.pdf}
\caption{Zoomed views of cloud mask results of FCD and FCD+ on scenes from each Biome.}
\label{fig:predictionszoom}
\end{figure*}

==> BigData 2021 Weakly-Supervised Cloud Detection with Fixed-Point GANs/figures/system.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{images/system.pdf}
\caption{Overview of FCD. We learn fixed-point translation between clear and cloudy image patches. During training, the discriminator $D$ learns to distinguish between real and fake images and to classify real images correctly. The generator $G$ is input an image and 
whether the image should be translated to the clear domain ($c=0$) or the cloudy domain ($c=1$), and learns to either remove or add clouds through a cycle-consistency loss and an adversarial loss. If $c$ is the same domain as the input image, $G$ must perform an identity mapping through the identity loss, which regularizes the generator to only affect the clouds. We then detect clouds in an input image $x$ by the difference between the original image and its clear translation with $G$.}
\label{fig:system}
\end{figure*}

==> BigData 2021 Weakly-Supervised Cloud Detection with Fixed-Point GANs/tables/hybrid_overall.tex <==
\begin{table}[t]
\caption{Cloud detection results for Landsat-8 Biome. The supervision type indicates: image-level labels $\mathcal{I}$, all available pixel-level labels $\mathcal{F}$, and 1\% of available pixel-level labels $\mathcal{F}^{1\%}$. Our proposed method achieves the highest performance with the least expensive labels.}
\centering
\begin{tabular}{llcc}
\toprule
Method                      & Supervision                     & F1-score              & Accuracy              \\
\midrule
CFmask \cite{foga2017biome} & -                               & 87.2                  & 87.7                  \\
\midrule
Random initialization       & $\mathcal{F}^{1\%}$             & 89.4$\pm$0.5          & 89.5$\pm$0.5          \\
Pretrained                  & $\mathcal{I}+\mathcal{F}^{1\%}$ & 91.5$\pm$0.4          & 91.6$\pm$0.4          \\
Fully supervised~\cite{Jeppesen2019} & $\mathcal{F}$                   & 93.9$\pm$0.5          & 94.0$\pm$0.5          \\
\midrule
FCD+ (ours)                    & $\mathcal{I}$                   & \textbf{91.5$\pm$0.6} & \textbf{91.7$\pm$0.6} \\
FCD+1\% (ours)                & $\mathcal{I}+\mathcal{F}^{1\%}$ & \textbf{93.4$\pm$0.5} & \textbf{93.5$\pm$0.4} \\
\bottomrule
\end{tabular}   
\label{table:hybridoverall}
\end{table}

==> BigData 2021 Weakly-Supervised Cloud Detection with Fixed-Point GANs/tables/pseudo_masks.tex <==
\begin{table}[t]
\caption{Cloud mask generation performance (\%) for Landsat-8 Biome with existing CAM methods and our FCD.}
\centering
\begin{tabular}{lcc}
    \toprule
    Method                                     & F1-score & Accuracy \\ \midrule
    CAM~\cite{zhou2016learning}                & 75.9$\pm$0.5                              & 82.9$\pm$0.7 \\
    GradCAM~\cite{selvaraju2017gradcam}        & 70.5$\pm$1.5                              & 78.6$\pm$0.5 \\
    GradCAM++~\cite{chattopadhay2018gradcampp} & 72.2$\pm$3.8                              & 79.9$\pm$1.9 \\
    \midrule
    FCD (ours)                                    & \textbf{83.9$\pm$0.8}                              & \textbf{87.6$\pm$0.5} \\
    \bottomrule
\end{tabular}
\label{table:fpganoverall}
\end{table}

==> figures/predictions_zoom.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\linewidth]{images/predictions_zoom.pdf}
\caption{Zoomed views of cloud mask results of FCD and FCD+ on scenes from each Biome.}
\label{fig:predictionszoom}
\end{figure*}
